Shape-Sensitive Loss for Catheter and Guidewire Segmentation

We introduce a shape-sensitive loss function for catheter and guidewire segmentation and utilize it in a vision transformer network to establish a new state-of-the-art result on a large-scale X-ray images dataset. We transform network-derived predictions and their corresponding ground truths into signed distance maps, thereby enabling any networks to concentrate on the essential boundaries rather than merely the overall contours. These SDMs are subjected to the vision transformer, efficiently producing high-dimensional feature vectors encapsulating critical image attributes. By computing the cosine similarity between these feature vectors, we gain a nuanced understanding of image similarity that goes beyond the limitations of traditional overlap-based measures. The advantages of our approach are manifold, ranging from scale and translation invariance to superior detection of subtle differences, thus ensuring precise localization and delineation of the medical instruments within the images. Comprehensive quantitative and qualitative analyses substantiate the significant enhancement in performance over existing baselines, demonstrating the promise held by our new shape-sensitive loss function for improving catheter and guidewire segmentation.

==> table-Coefficients.tex <==
\begin{table}[htbp]
\centering
\caption{Effects of Blending Parameters: \(\gamma\) for Dice Loss and \(\delta\) for Our Proposed Shape-Sensitive Loss on Various Network Architectures.}\label{table:coefficients}
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\textbf{Network}} & \multicolumn{2}{c}{\textbf{Coefficient}} & \multirow{2}{*}{\textbf{Dice Coefficient (\%)}} \\
& \textbf{$\gamma$} & \textbf{$\delta$} & \\ 
\midrule
\multirow{5}{*}{TransU-Net} & 0.1 & 0.9 & 56.68 \\  
& 0.3 & 0.7 & 57.03 \\  
& 0.5 & 0.5 & 57.16 \\  
& 0.7 & 0.3 & 56.91 \\  
& 0.9 & 0.1 & 56.89 \\ 
\midrule
\multirow{5}{*}{SwinU-Net} & 0.1 & 0.9 & 54.15 \\  
& 0.3 & 0.7 & 54.23 \\  
& 0.5 & 0.5 & 54.71 \\  
& 0.7 & 0.3 & 54.55 \\  
& 0.9 & 0.1 & 54.50 \\ 
\bottomrule
\end{tabular}
\end{table}

==> table-combinationOfLoss.tex <==
\begin{table}[htbp]
\centering
\caption{Performance Comparison of Different Loss Function Combinations Catheter and Guidewire Segmentation using Dice Coefficient.}\label{table:Combination}
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{Loss Function} & \textbf{Dice Coefficient (\%)} \\ 
\midrule
Cross-Entropy and Dice loss & 54.52 \\  
Focal Tversky and \textbf{\textcolor{blue}{ours}} & 55.78 \\ 
Combo and \textbf{\textcolor{blue}{ours}} & 56.63 \\ 
Dice and \textbf{\textcolor{blue}{ours}} & 57.16 \\  
\bottomrule
\end{tabular}
\end{table}

==> table-distance.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Dice Coefficients Achieved using Various Distance Measurements for Loss Value Calculation.}\label{table:Distance}
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{Distance Measurement} & \textbf{Dice Coefficient (\%)} \\ 
\midrule
Cosine similarity & 57.16 \\  
Euclidean distance & 56.78\\  
Manhattan distance (L1 Norm) & 56.10\\ 
Jaccard similarity & 56.72\\  
Hamming distance & 54.03\\  
\bottomrule
\end{tabular}
\end{table}

==> table-test.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[htbp]
    \centering
    \small
    \renewcommand{\thempfootnote}{\arabic{mpfootnote}}
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{Performance Comparison of Different Loss Function Combinations for Catheter and Guidewire Segmentation using Dice Coefficient.}\label{table:Combination}
        \begin{tabularx}{\linewidth}{@{}YY@{}}
            \toprule
            \textbf{Loss Function} & \textbf{Dice (\%)} \\
            \midrule
            CE\footnotemark[1] and Dice & 54.52 \\
            FT\footnotemark[2] and \textbf{\textcolor{blue}{ours}} & 55.78 \\
            Combo and \textbf{\textcolor{blue}{ours}} & 56.63 \\
            Dice and \textbf{\textcolor{blue}{ours}} & 57.16 \\
            \bottomrule
        \end{tabularx}
        \footnotetext[1]{CE = Cross-Entropy}
        \footnotetext[2]{FT = Focal Tversky}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{Effects of Blending Parameters: \(\gamma\) for Dice Loss and \(\delta\) for Our Proposed Shape-Sensitive Loss on Various Network Architectures.}\label{table:coefficients}
        \begin{tabularx}{\linewidth}{@{}Cccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Network}} & \multicolumn{2}{c}{\textbf{Coefficient}} & \multirow{2}{*}{\textbf{Dice (\%)}} \\
            & \textbf{$\gamma$} & \textbf{$\delta$} & \\ 
            \midrule
            \multirow{5}{*}{TransU-Net} & 0.1 & 0.9 & 56.68 \\  
            & 0.3 & 0.7 & 57.03 \\  
            & 0.5 & 0.5 & 57.16 \\  
            & 0.7 & 0.3 & 56.91 \\  
            & 0.9 & 0.1 & 56.89 \\ 
            \midrule
            \multirow{5}{*}{SwinU-Net} & 0.1 & 0.9 & 54.15 \\  
            & 0.3 & 0.7 & 54.23 \\  
            & 0.5 & 0.5 & 54.71 \\  
            & 0.7 & 0.3 & 54.55 \\  
            & 0.9 & 0.1 & 54.50 \\ 
            \bottomrule
        \end{tabularx}
    \end{minipage}
\end{table}
